Truth and Regret in Online Scheduling

We consider a scheduling problem where a cloud service provider has multiple units of a resource available over time. Selfish clients submit jobs, each with an arrival time, deadline, length, and value. The service provider's goal is to implement a truthful online mechanism for scheduling jobs so as to maximize the social welfare of the schedule. Recent work shows that under a stochastic assumption on job arrivals, there is a single-parameter family of mechanisms that achieves near-optimal social welfare. We show that given any such family of near-optimal online mechanisms, there exists an online mechanism that in the worst case performs nearly as well as the best of the given mechanisms. Our mechanism is truthful whenever the mechanisms in the given family are truthful and prompt, and achieves optimal (within constant factors) regret. We model the problem of competing against a family of online scheduling mechanisms as one of learning from expert advice. A primary challenge is that any scheduling decisions we make affect not only the payoff at the current step, but also the resource availability and payoffs in future steps. Furthermore, switching from one algorithm (a.k.a. expert) to another in an online fashion is challenging both because it requires synchronization with the state of the latter algorithm as well as because it affects the incentive structure of the algorithms. We further show how to adapt our algorithm to a non-clairvoyant setting where job lengths are unknown until jobs are run to completion. Once again, in this setting, we obtain truthfulness along with asymptotically optimal regret (within poly-logarithmic factors).

==> nctruth.tex <==
\subsection{Truthful switching in the non-clairvoyant setting}
\label{sec:nc-truth}
We recall some of the differences in a non-clairvoyant setting. 
A non-clairvoyant algorithm cannot plan for a complete schedule ahead of time, 
since the processing lengths are not known in advance. 
The algorithm maintains a queue of unfinished jobs and 
at every time $t$ decides which job to schedule from this queue at that time.
The deadline for a job is the number of time slots that the job is willing to wait out. 
If a job passes its deadline, which means that the number of time slots that a job $j$ waits since its arrival exceeds a threshold $d_j$, then the job is deleted from the queue. 
Due to this reason, the notion of promptness is not quite applicable to the non-clairvoyant setting. 
In its place, we use the  \orderresp property, which states that only jobs arriving earlier can influence the allocation and payments for a given job.
% attains a crucial role in the non-clairvoyant setting. 
We assume that there is a total order on the arrival time of the jobs, by breaking ties arbitrarily in case multiple jobs arrive at the same time. 


We treat a job influencing the mechanism to move it down the arrival order the same way as reporting a later arrival time: it cannot be benfecial to do this given that the mechanism is truthful. 
Exampes of mechanisms that are truthful and \orderresp are ``FIFO with fixed price'': 
	all jobs whose value is less than a threshold price are rejeceted, and the rest of the jobs are scheduled in the arrival order. 
Such mechanisms are close to optimal in a stochastic setting \citep{}. 

In the non-clairvoyant setting, we restart the algorithm at random, which is an event that takes place over an interval of duration $\dlmax$. 
The reason the restart is defined in a certain way (Definition \ref{def:random-restart}) is that this preserves the truthfulness property. We now prove this. 
\begin{lemma}\label{lem:truth-restart}
	{If $A$ is an order respecting truthful mechanism, then $A$ with (arbitrary) restarts is also order respecting and truthful. }
\end{lemma}
\begin{proof}
	We assume that $A$ is restarted in the interval $[1,\dlmax]$, and that the decision to restart is not dependent on what the jobs report.
	For a job that arrives by time 0, reporting an arrival time after 0 is not beneficial since that would mean that this job can only be processed beginning time $\dlmax+1$, and the job would be past its deadline by then. 
	If the job reports an arrival time before time 1, then truthfulness of $A$ guarantees that no misreport is beneficial. 
	
	Now consider a job $j$ that arrives after time 0. 
	If the deadline of this job is such that it has to start by time $\dlmax$, then no matter what it reports it does not get scheduled. 
	For all other jobs, consider the instance where the jobs that arrive during the interval $[1,\dlmax]$ actually arrive at time $\dlmax+1$, with the same arrival order. 
	Truthfulness of $A$ for this instance guarantees truthfulness for such jobs. 
	
\end{proof} 



The switching mechanism is based on a combination of ideas behind the switching mechanism for the clairvoyant case and the truthfulness of restarts in the non-clairvoyant case. 
The mechanism  $C$ is as follows. 
%We describe it in the clairvoyant setting. 
\begin{enumerate}
	\item For jobs that arrive by time $0$, mimic mechanism  $A$ and return the same allocation, schedule  and prices as $A$. 
	All these jobs are completed by time $\dlmax$. 
	\item For all remaining jobs, i.e., jobs $j$ with $a_j\geq 1$ run mechanism $B$ on these with the following modifications. 
	\begin{enumerate}            
		\item If the arrival time of a job is $< \dlmax$, set its arrival time to $\dlmax+1$. 
		\item Adjust the deadline of the job so that it reflects the time lost during the interval $[1,\dlmax]$. 
		This might mean some jobs are past their deadline. These jobs are rejected. 
		\item Preserve the arrival order. Use the tie breaking rule to make sure the arrival order of jobs whose starting time was set to $\dlmax$ is the same as in the original instance. 
	\end{enumerate}
\end{enumerate}


\begin{lemma}\label{lem:state-match}
	The state of the algorithm $C$ at time $\dlmax$ is the same as the state of the algorithm $B$ at time $\dlmax$, given that $B$ is restarted during the interval $[1,\dlmax]$.
\end{lemma}
\begin{proof} 
This follows by observing that Step (2) of mechanism 	$C$ is identical to the modifications made during a restart. 
Any job that arrives by time 0 does not influence the state of mechanism $B$ at time $\dlmax$ in either case. 
\end{proof}

\begin{lemma} \label{lem:truthfulswitching}
	Given \orderresp truthful mechanisms $A$ and $B$ in the non-clairvoyant setting, 
	mechanism $C$ as defined above is \orderresp, truthful, and obtains welfare at least 
	$$ \textstyle \sum_{t\le \dlmax} W_t(A) + \sum_{t\geq1 + \dlmax} W_t(B) ,$$ 
	given that $A$ and $B$ are restarted during the interval $[1,\dlmax]$.
	%The algorithm $C$ ``switches'' from running $A$ to running $B$ while maintaining truthfulness and without losing too much welfare.
\end{lemma} 
\begin{proof}
	The mechanism $C$ is \orderresp by definition. 
	Truthfulness of mechanism $C$ follows essentially from the truthfulness of restarts (Lemma~\ref{lem:truth-restart}). 
	For any job that arrives before time 1, reporting an arrival time $\geq 1$ is not beneficial since it would only begin processing after $\dlmax$ by which time its deadline would  have passed. 
	If it reports a time before 1, then the truthfulness of $A$ guarantees that no misreport can be beneficial. 
	For any job that arrives after time 0, the situation is exactly the same as a restart. What mechanism was run before time 1 has no bearing on the allocation and payments of this job.
	Lemma~\ref{lem:truth-restart} guarantees truthfulness for these jobs. 
	 
	 The welfare guarantee follows from observing that mechanism $C$ completes all jobs that mechanism $A$ started  before time 1, and 
	 that after time $\dlmax$, the welfare of $C$ matches that of  $B$ due to Lemma \ref{lem:state-match}. 
	 The only loss of welfare is in the interval $[1,\dlmax]$ which is bounded by $\vmax(\dlmax)$. 
	  
\end{proof} 
We can combine any number of switches just the way we do in Theorem \ref{thm:manyswitches}. 
%\end{document}

==> related.tex <==
\paragraph{\bf Related work}

The idea of combining several online algorithms into one that is
nearly as good as the best of them has been explored previously,
particularly in the context of metrical task systems and adaptive data
structures. See, e.g., \citet{BB00, BCK02}. To our knowledge, this
paper is the first to apply it to the context of online mechanisms. 

%Other scheduling mechanisms works: Azar and Khaitsin~\cite{azar2011prompt}


% 1. scheduling mechanisms and algorithms survey

% 2. This idea of combining several online algorithms into one that is
% nearly as good as the best of them is not novel -- it has been studied
% previously in purely algorithmic settings in the context of XXYYZZ. A
% primary challenge in adapting online learning approaches from the
% expert-advice setting to the algorithmic setting is that care needs to
% be taken in switching from one algorithm to another in the middle of
% the online process -- online algorithms carry state and it can be
% expensive to recreate the right state at the time of a switch, if at
% all possible.

% 3. experts+MAB literature




